Sub-Riemannian Ricci curvatures and universal diameter bounds for 3-Sasakian manifolds

For a fat sub-Riemannian structure, we introduce three canonical Ricci curvatures in the sense of Agrachev-Zelenko-Li. Under appropriate bounds we prove comparison theorems for conjugate lengths, Bonnet-Myers type results and Laplacian comparison theorems for the intrinsic sub-Laplacian. As an application, we consider the sub-Riemannian structure of $3$-Sasakian manifolds, for which we provide explicit curvature formulas. We prove that any complete $3$-Sasakian structure of dimension $4d+3$, with $d>1$, has sub-Riemannian diameter bounded by $\pi$. When $d=1$, a similar statement holds under additional Ricci bounds. These results are sharp for the natural sub-Riemannian structure on $\mathbb{S}^{4d+3}$ of the quaternionic Hopf fibrations: \begin{equation*} \mathbb{S}^3 \hookrightarrow \mathbb{S}^{4d+3} \to \mathbb{HP}^d, \end{equation*} whose exact sub-Riemannian diameter is $\pi$, for all $d \geq 1$.

==> prel.tex <==
\section{Sub-Riemannian geometry}

We give here only the essential ingredients for our analysis of sub-Riemannian structures arising from contract $3$-structures. For further details we refer to \cite{nostrolibro,montgomerybook}.

A sub-Riemannian structure $(\distr,g)$ on a manifold $M$ is given by a distribution $\distr \subset TM$ of constant rank, and a scalar product $g: \distr \times \distr \to \R$. This is a natural generalization of Riemannian geometry to take in account non-holonomic constraints. \emph{Admissible trajectories} are Lipschitz continuous curves $\gamma : [0,T] \to M$ that are tangent to the distribution.

We say that $\distr$ is \emph{bracket-generating} if the Lie algebra generated by sections of $\distr$, evaluated at any point of the manifold, is the whole tangent space:
\begin{equation}
\mathrm{Lie}(\distr)_q = T_q M, \qquad \forall q \in M.
\end{equation}
Admissible trajectories have a well defined \emph{sub-Riemannian length}
\begin{equation}
\ell(\gamma)= \int_{0}^T \|\dot\gamma(t)\| dt.
\end{equation}
The \emph{sub-Riemannian distance} $d:M \times M \to \R$ is
\begin{equation}
d(q,p):= \inf\{\ell(\gamma)\mid \gamma \text{ admissible joining $p$ with $q$}\}.
\end{equation}
By the Chow-Rashevskii theorem, under the bracket-generating condition, for any pair of points $q,p \in M$ there exists an admissible trajectory joining them and the metric topology induced by $d$ is the original one of $M$ (i.e. $d$ is finite and continuous). The definition of sub-Riemannian structure includes also Riemannian geometry, when $\distr = TM$.

\emph{Sub-Riemannian geodesics} are admissible curves that locally minimize the length between their endpoints. In our setting, all geodesics arise as solutions of an Hamiltonian system on $T^*M$. More precisely, define the \emph{sub-Riemannian Hamiltonian} $H : T^*M \to \R$ as
\begin{equation}
H(\lambda) := \frac{1}{2}\sum_{i=1}^k \langle \lambda, X_i \rangle^2, \qquad \lambda \in T^*M,
\end{equation}
where $X_1,\ldots,X_k$ is any local orthonormal frame for $\distr$ and $\langle \lambda, \cdot \rangle $ denotes the action of covectors on vectors. If $\sigma \in \Lambda^2 T^*M$ denotes the canonical symplectic $2$-form on $T^*M$, the \emph{Hamiltonian vector field} $\vec{H}$ is defined by $\sigma(\cdot, \vec{H}) = dH$. Then the Hamilton equations are
\begin{equation}\label{eq:Hamiltoneqs}
\dot{\lambda}(t) = \vec{H}(\lambda(t)).
\end{equation}
Solutions $\lambda : [0,1] \to T^*M$ of~\eqref{eq:Hamiltoneqs} are called \emph{extremals}, and their projections $\gamma(t) := \pi(\lambda(t))$, where $\pi :T^*M \to M$, are locally optimal admissible trajectories. In all cases we consider here, these are precisely all the sub-Riemannian geodesics. In particular, any curve realizing the distance between two points is a solution of \eqref{eq:Hamiltoneqs}. 

Clearly, an extremal (and thus a geodesic) depends on the choice of the initial covector $\lambda$. We define the \emph{sub-Riemannian exponential mapping} $\exp_{q} : T^*_q M \to M$, with base $q \in M$ as
\begin{equation}
\exp_q (\lambda) := \pi \circ e^{\vec{H}}(\lambda), \qquad \lambda \in T_q^*M,
\end{equation}
where the symbol $e^{t \vec{H}}(\lambda)$ denotes the solution of~\eqref{eq:Hamiltoneqs} (we assume $\vec{H}$ to be complete, i.e. all the extremals can be prolonged for all times). 

The speed of a geodesic $\|\dot\gamma(t)\|$ is constant and is equal to $2H(\lambda)$. Thus the set of initial covectors for unit speed geodesics starting at $q \in M$ is
\begin{equation}
\cyl_q  =\{\lambda  \in T_q^*M \mid  H(\lambda) = 1/2 \} \simeq \mathbb{S}^{k-1} \times \R^{n-k}.
\end{equation}
In the Riemannian case, $H|_{T_q^*M}$ is a positive definite quadratic form, and $\cyl_q$ is homeomorphic to a sphere. In the sub-Riemannian case, $H|_{T_q^*M} \geq 0$ but has rank $k < n$, hence $\cyl_q$ is homeomorphic to a cylinder.

For $\lambda \in \cyl_q$, the curve $\gamma_\lambda(t)=\exp_q(t \lambda)$ is a unit speed geodesic with length $\ell(\gamma|_{[0,T]}) = T$. We say that $t_*$ is a \emph{conjugate time} along $\gamma_\lambda$ if $t\lambda$ is a critical point of $\exp_q$. As it is well known in Riemannian geometry, the first conjugate time is separated from zero, and geodesics cease to be minimizing after the first conjugate time. This remains true for many sub-Riemannian structures and in particular for all the cases under investigation in this paper. 

The above statement is not true in full generality, as the presence of the so-called abnormal geodesics must be taken in account. These are poorly understood minimizing trajectories that might not follow the Hamiltonian dynamic of~\eqref{eq:Hamiltoneqs}.

\begin{rmk}
In the Riemannian case, due to the canonical identification $TM \simeq T^*M$, the exponential map defined above is just the ``dual'' of the standard exponential one. However the duality fails in the sub-Riemannian case, and only the ``cotangent'' viewpoint remains.
\end{rmk}

